JCloudScale: Closing the Gap Between IaaS and PaaS

The Infrastructure-as-a-Service (IaaS) model of cloud computing is a promising approach towards building elastically scaling systems. Unfortunately, building such applications today is a complex, repetitive and error-prone endeavor, as IaaS does not provide any abstraction on top of naked virtual machines. Hence, all functionality related to elasticity needs to be implemented anew for each application. In this paper, we present JCloudScale, a Java-based middleware that supports building elastic applications on top of a public or private IaaS cloud. JCloudScale allows to easily bring applications to the cloud, with minimal changes to the application code. We discuss the general architecture of the middleware as well as its technical features, and evaluate our system with regard to both, user acceptance (based on a user study) and performance overhead. Our results indicate that JCloudScale indeed allowed many participants to build IaaS applications more efficiently, comparable to the convenience features provided by industrial Platform-as-a-Service (PaaS) solutions. However, unlike PaaS, using JCloudScale does not lead to a loss of control and vendor lock-in for the developer.

==> scenario.tex <==
\section{Motivating Scenario}
\label{sec:scenario}

Consider \JSTaaS (``JavaScript Testing-as-a-Service''), the product of an
illustrative Web startup. \JSTaaS provides testing of JavaScript applications as a
cloud service.
Clients register with the service, which triggers \JSTaaS to periodically launch
this client's registered test suites. Results of test runs are stored in a
database, which can be queried by the client. Tests vary widely in the load that
they generate on the servers, and clients are billed according to this load.
% \JSTaaS should be implemented as a Java-based application.
% A very rough architecture sketch of the application is given in
% Figure~\ref{fig:scenario}.

% \begin{figure}[h!]
% \centering
% \includegraphics[width=0.85\linewidth]{img/scenario}
%   \caption{DRAFT - \JSTaaS Illustrative Example}
%   \label{fig:scenario}
% \end{figure}

As the startup has limited initial funding, it has been decided that the initial
version of \JSTaaS should be deployed as a Java-based service on Amazon's EC2
public IaaS cloud, so that infrastructure costs
will only grow in line with actual demand. Furthermore, to save costs, virtual
machines, which will be used to launch actual tests, should be utilized to the
highest degree possible. This means that tests should be co-located on the same
virtual machines as far as possible, and idle machines should be released if
they are not required any longer. To this end, the core of \JSTaaS needs to
continuously monitor the utilization of all hosts, as well as the execution time
of tests, in order to decide which hosts to keep online and which to tear down.

Using standard tools, this application is not trivial to implement. Developers
need to split the application into task manager, load balancer and workers to
execute the tests, setup virtual machines, install the respective application
components on these virtual machines and, at runtime, monitor to make sure that
the application is not over- or under-provisioned. Tools such as AWS Elastic
Beanstalk (deployment) or CloudWatch (monitoring) can be used to ease these
tasks to some extent. However, even using these advanced tools, cloud deployment
quickly becomes a labor-intensive chore. Hence, the startup decides to use the
\cs middleware to build \JSTaaS. The startup hopes that \cs will help its few
developers to efficiently write this elastic application, and devise good
scaling and scheduling policies. Furthermore, the integrated event-based
monitoring of \cs will also be useful for customer billing. Finally, building
their application on top of the \cs abstraction allows the startup to easily
migrate their application, e.g., to an OpenStack based private cloud, should
they decide to move away from Amazon EC2 in the future.

